High-Reynolds-number turbulent boundary layers under adverse pressure gradients. Part 2. A composite mean velocity profile

A robust composite mean velocity profile is developed for turbulent boundary layers (TBLs) subjected to adverse pressure gradients (APGs), extending the composite formulation for generic pressure-gradient TBLs proposed by \citeauthor{nickels} (\textit{J.\ Fluid Mech.}, vol.\ 521, 2004). Several modifications are introduced to capture key features of APG flows. A new parameter accounts for pressure-gradient history effects in the wake region, a velocity-overshoot function is incorporated in the inner region, and the wake function is reformulated using an independent, physically motivated definition of boundary-layer thickness. A compilation of APG TBL datasets from the literature, including the new dataset presented in Part~1, is used to assess and refine the formulation. The resulting composite profile contains three physically meaningful parameters that capture pressure-gradient effects on the mean velocity profile, determined through nonlinear curve fitting. These parameters provide a framework for identifying `well-behaved' APG TBLs and quantifying the strength of pressure-gradient history effects. The profile also enables reliable estimation of the friction velocity and boundary-layer thickness in well-behaved APG TBLs, providing a practical tool for scaling analyses when these quantities are not directly measurable. Its analytical form yields improved estimates of mean velocity gradients, facilitating evaluation of the indicator function and identification of inflection points. Finally, the formulation predicts both the coefficients and spatial extent of the logarithmic region of the mean streamwise velocity profile, enabling assessment of its universality in high-Reynolds-number APG TBLs. This shows that the von K'arm'an coefficient approaches an invariant value of $\kappa \approx 0.39$ at sufficiently high Reynolds numbers, independent of pressure-gradient effects.

==> references.tex <==
@article{coles1956law,
  title={The law of the wake in the turbulent boundary layer},
  author={Coles, D.},
  journal={J. Fluid Mech.},
  volume={1},
  number={2},
  pages={191--226},
  year={1956}
}

@article{Monkewitz_Nagib_2023, title={The hunt for the {K}ármán ‘constant’ revisited}, volume={967}, DOI={10.1017/jfm.2023.448}, journal={J. Fluid Mech.}, author={Monkewitz, P. A. and Nagib, H. M.}, year={2023}, pages={A15}}

@article{nagano,
  title={Structure of turbulent boundary layer subjected to adverse pressure gradient},
  author={Nagano, Y. and Tsuji, T. and Houra, T.},
  journal={Int. J. Heat Fluid Flow},
  volume={19},
  number={5},
  pages={563--572},
  year={1998}
}

@article{deshpande,
  title={{R}eynolds-number effects on the outer region of adverse-pressure-gradient turbulent boundary layers},
  author={Deshpande, R. and Van Den Bogaard, A. and Vinuesa, R. and Lindi{\'c}, L. and Marusic, I.},
  journal={Phys. Rev. Fluids},
  volume={8},
  number={12},
  pages={124604},
  year={2023}
}

@article{harun,
  title={Pressure gradient effects on the large-scale structure of turbulent boundary layers},
  author={Harun, Z. and Monty, J. P. and Mathis, R. and Marusic, I.},
  journal={J. Fluid Mech.},
  volume={715},
  pages={477--498},
  year={2013}
}

@article{bobke2017history,
  title={History effects and near equilibrium in adverse-pressure-gradient turbulent boundary layers},
  author={Bobke, A. and Vinuesa, R. and {\"O}rl{\"u}, R. and Schlatter, P.},
  journal={J. Fluid Mech.},
  volume={820},
  pages={667--692},
  year={2017}
}

@article{pozuelo,
  title={An adverse-pressure-gradient turbulent boundary layer with nearly constant $\beta \simeq 1.4$ up to ${R}e_{\theta } \simeq 8700$},
  author={Pozuelo, R. and Li, Q. and Schlatter, P. and Vinuesa, R.},
  journal={J. Fluid Mech.},
  volume={939},
  pages={A34},
  year={2022}
}
@article{romero202history,
  title={Velocity spectra and scale decomposition of adverse pressure gradient turbulent boundary layers considering history effects},
  author={Romero, S. and Zimmerman, S. and Philip, J. and Klewicki, J.},
  journal={Int. J. Heat Fluid Flow},
  volume={102},
  pages={109143},
  year={2023}
}

@article{romero2022,
  title={Properties of the inertial sublayer in adverse pressure-gradient turbulent boundary layers},
  author={Romero, S. and Zimmerman, S. and Philip, J. and White, C. and Klewicki, J.},
  journal={J. Fluid Mech.},
  volume={937},
  pages={A30},
  year={2022}
}

@article{vaquero,
  title={Effects of upstream perturbations on the solution of the laminar and fully turbulent boundary layer equations with pressure gradients},
  author={Vaquero, J. and Renard, N. and Deck, S.},
  journal={Phys. Fluids},
  volume={31},
  number={12},
  year={2019}
}

@article{vinuesa2017revisiting,
  title={Revisiting history effects in adverse-pressure-gradient turbulent boundary layers},
  author={Vinuesa, R. and {\"O}rl{\"u}, R. and Sanmiguel Vila, C. and Ianiro, A. and Discetti, S. and Schlatter, P.},
  journal={Flow Turbul. Combust.},
  volume={99},
  pages={565--587},
  year={2017}
}

@article{vila2020,
  title={Experimental realisation of near-equilibrium adverse-pressure-gradient turbulent boundary layers},
  author={Sanmiguel Vila, C. and Vinuesa, R. and Discetti, S. and Ianiro, A. and Schlatter, P. and {\"O}rl{\"u}, R.},
  journal={Exp. Therm. Fluid Sci.},
  volume={112},
  pages={109975},
  year={2020}
}

@article{vila2017,
  title={On the identification of well-behaved turbulent boundary layers},
  author={Sanmiguel Vila, C. and Vinuesa, R. and Discetti, S. and Ianiro, A. and Schlatter, P. and {\"O}rl{\"u}, R.},
  journal={J. Fluid Mech.},
  volume={822},
  pages={109--138},
  year={2017},
  publisher={Cambridge University Press}
}

@article{clauser1954turbulent,
  title={Turbulent boundary layers in adverse pressure gradients},
  author={Clauser, F. H.},
  journal={J. Aeronaut. Sci.},
  volume={21},
  number={2},
  pages={91--108},
  year={1954}
}

@article{volino2020non,
  title={Non-equilibrium development in turbulent boundary layers with changing pressure gradients},
  author={Volino, R. J.},
  journal={J. Fluid Mech.},
  volume={897},
  pages={A2},
  year={2020}
}

@article{smits2011high,
  title={High--{R}eynolds number wall turbulence},
  author={Smits, A. J. and McKeon, B. J. and Marusic, I.},
  journal={Annu. Rev. Fluid Mech.},
  volume={43},
  number={1},
  pages={353--375},
  year={2011}
}

@article{smits2022batchelor,
  title={Batchelor Prize Lecture: Measurements in wall-bounded turbulence},
  author={Smits, A. J.},
  journal={J. Fluid Mech.},
  volume={940},
  pages={A1},
  year={2022}
}

@article{nickels,
  title={Inner scaling for wall-bounded flows subject to large pressure gradients},
  author={Nickels, T. B.},
  journal={J. Fluid Mech.},
  volume={521},
  pages={217--239},
  year={2004}
}

@article{lee2009structures,
  title={Structures in turbulent boundary layers subjected to adverse pressure gradients},
  author={Lee, J.-H. and Sung, H. J.},
  journal={J. Fluid Mech.},
  volume={639},
  pages={101--131},
  year={2009}
}

@article{knopp2021experimental,
 title={Experimental analysis of the log law at adverse pressure gradient},
  author={Knopp, T. and Reuther, N. and Novara, M. and Schanz, D. and Sch{\"u}lein, E. and Schr{\"o}der, A. and K{\"a}hler, C. J.},
  journal={J. Fluid Mech.},
  volume={918},
  pages={A17},
  year={2021}
}

@article{clauser1956turbulent,
  title={The turbulent boundary layer},
  author={Clauser, F. H.},
  journal={Adv. Appl. Mech.},
  volume={4},
  pages={1--51},
  year={1956}
}

@article{drozdz2020description,
  title={A description of turbulence intensity profiles for boundary layers with adverse pressure gradient},
  author={Dr{\'o}{\.z}d{\.z}, A. and Elsner, W. and Niegodajew, P. and Vinuesa, R. and {\"O}rl{\"u}, R. and Schlatter, P.},
  journal={Eur. J. Mech. B Fluids},
  volume={84},
  pages={470--477},
  year={2020}
}

@article{chauhan2009criteria,
  title={Criteria for assessing experiments in zero pressure gradient boundary layers},
  author={Chauhan, K. A. and Monkewitz, P. A. and Nagib, H. M.},
  journal={Fluid Dyn. Res.},
  volume={41},
  number={2},
  pages={021404},
  year={2009}
}

@inproceedings{chauhan2007composite,
 title={On the composite logarithmic profile in zero pressure gradient turbulent boundary layers},
  author={Chauhan, K. and Nagib, H. and Monkewitz, P.},
  booktitle={45th AIAA Aerospace Sciences Meeting and Exhibit},
  pages={532},
  year={2007}
}

@article{van1956Profile,
  title={On turbulent flow near a wall},
  author={Van Driest, E. R.},
  journal={J. Aeronaut. Sci.},
  volume={23},
  number={11},
  pages={1007--1011},
  year={1956}
}

@article{van1963boundary,
  title={Boundary layer transition-freestream turbulence and pressure gradient effects},
  author={Van Driest, E. R. and Blumer, C. B.},
  journal={AIAA J.},
  volume={1},
  number={6},
  pages={1303--1306},
  year={1963}
}

@article{hutchins2009hot,
  title={Hot-wire spatial resolution issues in wall-bounded turbulence},
  author={Hutchins, N. and Nickels, T. B. and Marusic, I. and Chong, M. S.},
  journal={J. Fluid Mech.},
  volume={635},
  pages={103--136},
  year={2009}
}

@article{spalding1961single,
  title={A single formula for the law of the wall},
  author={Spalding, D. B.},
  journal={J. Appl. Mech.},
  volume={28},
  number={3},
  pages={455--458},
  year={1961}
}

@article{orlu2010,
  title={On near wall measurements of wall bounded flows—the necessity of an accurate determination of the wall position},
  author={{\"O}rl{\"u}, R. and Fransson, J. H. M. and Alfredsson, P. H.},
  journal={Prog. Aerosp. Sci.},
  volume={46},
  number={8},
  pages={353--387},
  year={2010}
}

@article{musker1979explicit,
  title={Explicit expression for the smooth wall velocity distribution in a turbulent boundary layer},
  author={Musker, A. J.},
  journal={AIAA J.},
  volume={17},
  number={6},
  pages={655--657},
  year={1979}
}

@article{maciel2018outer,
  title={Outer scales and parameters of adverse-pressure-gradient turbulent boundary layers},
  author={Maciel, Y. and Wei, T. and Gungor, A. G. and Simens, M. P.},
  journal={J. Fluid Mech.},
  volume={844},
  pages={5--35},
  year={2018}
}

@article{krug2017,
  title={Revisiting the law of the wake in wall turbulence},
  author={Krug, D. and Philip, J. and Marusic, I.},
  journal={J. Fluid Mech.},
  volume={811},
  pages={421--435},
  year={2017}
}

@article{gomez2025his,
  title={Linear analysis characterizes pressure gradient history effects in turbulent boundary layers},
  author={Gomez, S. R. and McKeon, B. J.},
  journal={J. Fluid Mech.},
  volume={1002},
  pages={A20},
  year={2025}
}

@article{elnahhas2022momentom,
  title={On the enhancement of boundary layer skin friction by turbulence: an angular momentum approach},
  author={Elnahhas, A. and Johnson, P. L.},
  journal={J. Fluid Mech.},
  volume={940},
  pages={A36},
  year={2022}
}

@article{han2024outer,
  title={Consistent outer scaling and analysis of adverse pressure gradient turbulent boundary layers},
  author={Han, M. and Ma, M. and Yan, C.},
  journal={J. Fluid Mech.},
  volume={982},
  pages={A17},
  year={2024}
}

@article{jones2001sink,
  title={Evolution and structure of sink-flow turbulent boundary layers},
  author={Jones, M. B. and Marusic, I. and Perry, A. E.},
  journal={J. Fluid Mech.},
  volume={428},
  pages={1--27},
  year={2001}
}

@article{cantwell2022,
  title={A new boundary layer integral method based on the universal velocity profile},
  author={Cantwell, B. J. and Bilgin, E. and Needels, J. T.},
  journal={Phys. Fluids},
  volume={34},
  number={7},
  year={2022}
}

@article{yoon,
  title={Contribution of large-scale motions to the skin friction in a moderate adverse pressure gradient turbulent boundary layer},
  author={Yoon, M. and Hwang, J. and Sung, H. J.},
  journal={J. Fluid Mech.},
  volume={848},
  pages={288--311},
  year={2018}
}

@article{orlu2013,
  title={Comparison of experiments and simulations for zero pressure gradient turbulent boundary layers at moderate {R}eynolds numbers},
  author={{\"O}rl{\"u}, R. and Schlatter, P.},
  journal={Exp. Fluids},
  volume={54},
  pages={1--21},
  year={2013}
}

@article{monty2011,
  title={A parametric study of adverse pressure gradient turbulent boundary layers},
  author={Monty, J. P. and Harun, Z. and Marusic, I.},
  journal={Int. J. Heat Fluid Flow},
  volume={32},
  number={3},
  pages={575--585},
  year={2011}
}

@article{subrahmanyam2022integral,
  title={A universal velocity profile for turbulent wall flows including adverse pressure gradient boundary layers},
  author={Subrahmanyam, M. A. and Cantwell, B. J. and Alonso, J. J.},
  journal={J. Fluid Mech.},
  volume={933},
  pages={A16},
  year={2022}
}

@article{maruvsic1995wall,
  title={A wall-wake model for the turbulence structure of boundary layers. {P}art 2. Further experimental support},
  author={Marusic, I. and Perry, A. E.},
  journal={J. Fluid Mech.},
  volume={298},
  pages={389--407},
  year={1995}
}

@article{gungor2024,
  title={Turbulent boundary layer response to uniform changes of the pressure force contribution},
  author={Gungor, T. R. and Gungor, A. G. and Maciel, Y.},
  journal={J. Fluid Mech.},
  volume={997},
  pages={A75},
  year={2024}
}

@article{eitel2014simulation,
  title={Simulation and validation of a spatially evolving turbulent boundary layer up to ${R}e_\theta$= 8300},
  author={Eitel-Amor, G. and {\"O}rl{\"u}, R. and Schlatter, P.},
  journal={Int. J. Heat Fluid Flow},
  volume={47},
  pages={57--69},
  year={2014}
}

@article{monkewitz2007self,
  title={Self-consistent high-{R}eynolds-number asymptotics for zero-pressure-gradient turbulent boundary layers},
  author={Monkewitz, P. A. and Chauhan, K. A. and Nagib, H. M.},
  journal={Phys. Fluids},
  volume={19},
  number={11},
  year={2007}
}

@article{monkewitz2021late,
  title={The late start of the mean velocity overlap log law at--a generic feature of turbulent wall layers in ducts},
  author={Monkewitz, P. A.},
  journal={J. Fluid Mech.},
  volume={910},
  pages={A45},
  year={2021}
}

@article{wei2005properties,
  title={Properties of the mean momentum balance in turbulent boundary layer, pipe and channel flows},
  author={Wei, T. and Fife, P. and Klewicki, J. and McMurtry, P.},
  journal={J. Fluid Mech.},
  volume={522},
  pages={303--327},
  year={2005}
}

@article{klewicki2013,
  title={A description of turbulent wall-flow vorticity consistent with mean dynamics},
  author={Klewicki, J. C.},
  journal={J. Fluid Mech.},
  volume={737},
  pages={176--204},
  year={2013}
}

@article{fife2005stress,
  title={Stress gradient balance layers and scale hierarchies in wall-bounded turbulent flows},
  author={Fife, P. and Wei, T. and Klewicki, J. and McMurtry, P.},
  journal={J. Fluid Mech.},
  volume={532},
  pages={165--189},
  year={2005}
}

@article{vinuesa2016delta,
  title={On determining characteristic length scales in pressure-gradient turbulent boundary layers},
  author={Vinuesa, R. and Bobke, A. and {\"O}rl{\"u}, R. and Schlatter, P.},
  journal={Phys. Fluids},
  volume={28},
  number={5},
  year={2016}
}

@article{lozier2025defining,
  author  = {Lozier, M. and Deshpande, R. and Zarei, A. and Lindi{\'c}, L. and Rowin, W. A. and Marusic, I.},
  title   = {Defining the mean turbulent boundary layer thickness based on streamwise velocity skewness},
  journal = {J. Fluid Mech.},
  volume  = {1021},
  pages   = {A19},
  year    = {2025}
}

@article{marusic2015,
  title={Evolution of zero-pressure-gradient boundary layers from different tripping conditions},
  author={Marusic, I. and Chauhan, K. A. and Kulandaivelu, V. and Hutchins, N.},
  journal={J. Fluid Mech.},
  volume={783},
  pages={379--411},
  year={2015}
}

@article{marusic2010wall,
  title={Wall-bounded turbulent flows at high {R}eynolds numbers: recent advances and key issues},
  author={Marusic, I. and McKeon, B. J. and Monkewitz, P. A. and Nagib, H. M. and Smits, A. J. and Sreenivasan, K. R.},
  journal={Phys. Fluids},
  volume={22},
  number={6},
  year={2010}
}

@book{tennekes1972first,
 title={A first course in turbulence},
  author={Tennekes, H. and Lumley, J. L.},
  year={1972},
  publisher={MIT Press}
}

@article{nagib2008,
  title={Variations of von K{\'a}rm{\'a}n coefficient in canonical flows},
  author={Nagib, H. M. and Chauhan, K. A.},
  journal={Phys. Fluids},
  volume={20},
  number={10},
  year={2008}
}

@article{nagib2024method,
  title={A method for evaluating relations of turbulent normal-stresses by experimental data over a wide range of {R}eynolds numbers},
  author={Nagib, H. and Marusic, I.},
   journal={J. Fluid Mech.},
  volume={1016},
  pages={A24},
  year={2025},
}

@article{waltz2006,
  title={An interior algorithm for nonlinear optimization that combines line search and trust region steps},
  author={Waltz, R. A. and Morales, J. L. and Nocedal, J. and Orban, D.},
  journal={Math. Program.},
  volume={107},
  number={3},
  pages={391--408},
  year={2006}
}

@inproceedings{marusic2024turbulent,
  title={Turbulent/non-turbulent interface in high {R}eynolds number pressure gradient boundary layers},
  author={Marusic, I. and Abu Rowin, W. and Lozier, M. and Lindi{\'c}, L. and Zarei, A. and Deshpande, R.},
  booktitle={IUTAM Symposium on Turbulent/Non-Turbulent Interface in Turbulent Shear Flows},
  pages={3--17},
  year={2024}
}

@article{marusic2013logarithmic,
  title={On the logarithmic region in wall turbulence},
  author={Marusic, I. and Monty, J. P. and Hultmark, M. and Smits, A. J.},
  journal={J. Fluid Mech.},
  volume={716},
  pages={R3},
  year={2013}
}

@article{schlatter_turbulent_2012,
  title={Turbulent boundary layers at moderate {R}eynolds numbers: inflow length and tripping effects},
  author={Schlatter, P. and {\"O}rl{\"u}, R.},
  journal={J. Fluid Mech.},
  volume={710},
  pages={5--34},
  year={2012}
}

@article{perry_streamwise_2002,
    title={On the streamwise evolution of turbulent boundary layers in arbitrary pressure gradients},
  author={Perry, A. E. and Marusic, I. and Jones, M. B.},
  journal={J. Fluid Mech.},
  volume={461},
  pages={61--91},
  year={2002}
}

@article{li2021experimental,
  title={Experimental study of a turbulent boundary layer with a rough-to-smooth change in surface conditions at high {R}eynolds numbers},
  author={Li, M. and De Silva, C. M. and Chung, D. and Pullin, D. I. and Marusic, I. and Hutchins, N.},
  journal={J. Fluid Mech.},
  volume={923},
  pages={A18},
  year={2021}
}

@article{hutchins2007large,
  title={Large-scale influences in near-wall turbulence},
  author={Hutchins, N. and Marusic, I.},
  journal={Phil. Trans. R. Soc. A},
  volume={365},
  number={1852},
  pages={647--664},
  year={2007}
}

@article{preskett2025effects,
  title={Effects of pressure-gradient histories on skin friction and mean flow of high {R}eynolds number turbulent boundary layers over smooth and rough walls},
  author={Preskett, T. and Virgilio, M. and Jaiswal, P. and Ganapathisubramani, B.},
  journal={J. Fluid Mech.},
  volume={1010},
  pages={A30},
  year={2025}
}

@article{zarei2025decoupling,
  title={Decoupling pressure gradient history effects in turbulent boundary layers through high-{R}eynolds number experiments},
  author={Zarei, A. and Lozier, M. and Deshpande, R. and Marusic, I.},
  journal={arXiv preprint arXiv:2509.07545},
  year={2026}
}
@article{zarei2026_part1,
  title={High-{R}eynolds-number turbulent boundary layers under adverse pressure gradients. {P}art1. {D}ecoupling pressure gradient history effects},
  author={Zarei, A. and Lozier, M. and Deshpande, R. and Marusic, I.},
  journal={J. Fluid Mech. },
  note={Under review, arXiv preprint arXiv:2509.07545},
  year={2026}
}

@article{nagib2024utilizing,
  title={Utilizing indicator functions with computational data to confirm nature of overlap in normal turbulent stresses: Logarithmic or quarter-power},
  author={Nagib, H. and Vinuesa, R. and Hoyas, S.},
  journal={Phys. Fluids},
  volume={36},
  number={7},
  year={2024},
}

@article{chen2023,
  author  = {P. E. S. Chen and W. Wu and K. P. Griffin and Y. Shi and X. I. A. Yang},
  title   = {A universal velocity transformation for boundary layers with pressure gradients},
  journal = {J. Fluid Mech.},
  volume  = {970},
  pages   = {A3},
  year    = {2023}
}

@article{shu2025mean,
  title={Mean velocity profiles and total shear stress profiles in adverse-pressure-gradient turbulent boundary layers considering history effect},
  author={Shu, Z. and Xu, C.},
  journal={arXiv preprint arXiv:2508.07663},
  year={2025}
}

@article{yang2024,
  author  = {Yang, X. I. A. and Chen, P. E. S. and Zhang, W. and Kunz, R.},
  title   = {Predictive near-wall modelling for turbulent boundary layers with arbitrary pressure gradients},
  journal = {J. Fluid Mech.},
  volume  = {993},
  pages   = {A1},
  year    = {2024}
}

@article{panton2005,
  author  = {Panton, R. L.},
  title   = {Review of wall turbulence as describedd by composite expansions},
  journal = {App. Mech. Rev.},
  volume  = {58},
  pages   = {1--36},
  year    = {2005},
  doi = {10.1115/1.1840903}
}

@inproceedings{millikan1938,
  author  = {Millikan, C.},
  title   = {A critical discussion of turbulent flows in channels and circular tubes},
  booktitle = {Proc. 5th Int. Cong. Appl. Mech.},
  pages = {386--392},
  year = {1938},
}

@article{sharma2013coherent,
  title={On coherent structure in wall turbulence},
  author={Sharma, A. S. and McKeon, B. J.},
  journal={J. Fluid Mech.},
  volume={728},
  pages={196--238},
  year={2013},
}
@article{mesolayer,
  title={Experimental evidence for the existence of the ‘mesolayer’ in turbulent systems},
  author={Long, R. R. and Chen, T-C.},
 journal={J. Fluid Mech.},
  volume={105},
  pages={19--59},
  year={1981},
}

@article{woodcock2015statistical,
  title        = {The statistical behaviour of attached eddies},
  author       = {Woodcock, J.~D. and Marusic, I.},
  journal      = {Phys. Fluids},
  volume       = {27},
  number       = {1},
  year         = {2015}
}

@article{schatzman2017experimental,
  title   = {An experimental investigation of an unsteady adverse pressure gradient turbulent boundary layer: embedded shear layer scaling},
  author  = {Schatzman, D. M. and Thomas, F. O.},
  journal = {J. Fluid Mech.},
  volume  = {815},
  pages   = {592--642},
  year    = {2017}
}
